A Rewriting Theory for Quantum Lambda-Calculus

Quantum lambda calculus has been studied mainly as an idealized programming language -- the evaluation essentially corresponds to a deterministic abstract machine. Very little work has been done to develop a rewriting theory for quantum lambda calculus. Recent advances in the theory of probabilistic rewriting give us a way to tackle this task with tools unavailable a decade ago. Our primary focus is standardization and normalization results.

==> 01_Tables.tex <==



==> 03_Standardization.tex <==
%!TEX root = Main_quantum.tex	




==> 05_Expression.tex <==
%!TEX root = Main_Quantum.tex	



 
\section{Langrage of Benoît Valiron and Peter Selinger}
\todo{What is the role of this section??  Can we SUPPRESS?}


\begin{Def}
	This is the language of Benoît Valiron and Peter Selinger :
	\begin{align*}
		qTerm \; M,N,P  ::=&  x  \mid M N \mid  \lambda x . M \mid if \; M \; then \; N \; else \; P \mid
		0   \mid 	1 \mid meas \mid \\
		&	 new \mid U \mid \star \mid \pair{M}{N} \mid let \; \pair{x}{y}:= M \; in \; N
	\end{align*}
\end{Def}

\begin{Def}
	This is the language types of Benoît Valiron and Peter Selinger :
	\begin{align*}
		qType \; A,B ::=&  \bang^n \alpha  \mid \bang^n X \mid \bang^n (A \arrowrow B) \mid \bang^n \true \mid \bang^n (A \otimes B)
	\end{align*}
\end{Def}

\begin{notation}
	In order to simplify the notation, we will often use the following convention: we use pi to denote the free variable x such that $L(x) = i$. A program $[Q,L,M]$ is abbreviated to $[Q,M']$ with $M' = M[p_{i_1}/x_1] . . . [p_{i_n}/x_n]$, where $i_k = L(x_k)$.
	
	We have :
	\begin{itemize}
		\item $\bang^0 M = M.$
		\item $\bang^{n+1} M = \bang \bang^{n} M$
	\end{itemize} 
	
	We note $U_A$ for the term $U$ such that A is the matrix that define this quantum gate.
\end{notation}

\begin{Def}
	We define the function $\termtotermf : qTerm \times qType \rightarrow \QLambda$ by :
	\begin{itemize}
		\item $\termtoterm{x : \bang^n A} = !^{n} x$
		\item $\termtoterm{\lambda x . M :  \bang^n (A \arrowrow B) } = 
		\left\{\begin{matrix}
			\blam x . \termtoterm{M : B} \mbox{ if } B = \bang C\\ 
			\lam x . \termtoterm{M : B}\mbox{ else}
		\end{matrix}\right.$
		\item $\termtoterm{0 : \bang bit} = \lam f . \lam x . x$
		\item $\termtoterm{1 : \bang bit} = \lam f . \lam x . f x$
		\item $\termtoterm{new : \bang (bit \arrowrow qbit)} = \lam x . x U_{NOT} \new$
		\item $\termtoterm{meas : \bang (qbit \arrowrow \bang bit)} = \lam z . \meas{z}{\termtoterm{0 : \bang bit}}{\termtoterm{1 : \bang bit}}$
		\item $\termtoterm{if \; M \; then \; N \; else \; P : A} = \meas{\termtoterm{M : bit} \new}{\termtoterm{N : A}}{\termtoterm{P : A}}$
		\item $\termtoterm{U_A : \bang (qbit^n \arrowrow qbit^n)} = U_{A}$
		\item $\termtoterm{let \; \pair{x}{y}:= M \; in \; N : A} = \termtoterm{M : B} \lam x . \lam y . \termtoterm{N : A}$ avec $M : B$.
		\item $\termtoterm{M \; N : C} = \termtoterm{M : A}\termtoterm{N : B}$ avec $M : A$ et $N : B$.
		\item $\termtoterm{\pair{M}{N} : \bang^n (A_1 \otimes A_2)} = \termPair{f}{\termtoterm{M : \bang^n A_1}}{\termtoterm{N : \bang^n A_2}}$
		\item $\termtoterm{\star : \bang^n \true} = \lam x . x$
	\end{itemize}
\end{Def}

\begin{Def}
	Voici le terme $discard r_i = \meas{r_i}{I}{I}$
\end{Def}

\RED{
\begin{rem}[Measure problem]
	Our calculus doesn't allow us to lose a register.
	So how can we choose between one and an other ?
	For exemple, if we want to applicate the quantum gate NOT on $r_{1}$ or $r_{2}$ ?
	We can't directly because a term like that $\meas{r_0}{U_{NOT} r_{1}}{U_{NOT} r_{2}}$ isn't allowed (not the same registers in the branches of meas).
	But we can simulate this behavior with a term like that :
	\[ \meas{r_{0}}{\meas{r_{2}}{U_{NOT} r_{1}}{U_{NOT} r_{1}}}{\meas{r_{1}}{U_{NOT} r_{2}}{U_{NOT} r_{2}}} \]
\end{rem}
}

\begin{lem}
	(maybe more hypothesis)Assume $a$, $b$, $x$ are variables, $M$, $N$ are correct terms, $x$ is linear in $M$, $x$ is linear in $N$, $\Reg{M}=\Reg{N} = \emptyset$, then $\longmeasone{a}{b}{M}{N}$ is a correct term.
\end{lem}

\begin{lem}
	(maybe more hypothesis)Assume $a$, $b$, $x$ are variables, $M$, $N$ are correct terms, $a$,$b$ are linear in $M$, $a$,$b$ are linear in $N$, $\Reg{M}=\Reg{N} = \emptyset$, $i \neq j \neq k$ then $\longmeastwo{r_i}{r_j}{r_k}{M}{N}$ is a correct term.
\end{lem}

\begin{cor}
	\[\choicebetween{r_1}{r_2}{r_0}\] is a correct term.
\end{cor}

\paragraph{Expressiveness.}
If we reduce the last term, we can "choose" to keep the register 1 or the register 2 (it depends how register 0 is ponderated).

\begin{example}
	Let's reduce the previous term :
	\scriptsize{$
		\pair{Q}{\choicebetween{r_1}{r_2}{r_0}} \\
		\sfull \mdist{\prob{0}{0}{Q}\pair{Q_{0}}{(\blam f . f r_1 r_2 ) !\lam a . \lam b . (\longmeasone{a}{b}{x}{x})}, \\ \prob{1}{0}{Q}\pair{Q_{1}}{(\blam f . f r_1 r_2 ) !\lam a . \lam b . (\longmeasone{b}{a}{x}{x})}} \\
		\sfull \mdist{\prob{0}{0}{Q}\pair{Q_{0}}{\lam a . \lam b . (\longmeasone{a}{b}{x}{x})} r_1 r_2, \\ 
			\prob{1}{0}{Q}\pair{Q_{1}}{\lam a . \lam b . (\longmeasone{b}{a}{x}{x}) r_1 r_2}} \\
		\sfull \mdist{\prob{0}{0}{Q}\pair{Q_{0}}{\lam b . (\longmeasone{r_1}{b}{x}{x})} r_2, \\
			\prob{1}{0}{Q}\pair{Q_{1}}{\lam b . (\longmeasone{b}{r_1}{x}{x}) r_2}} \\
		\sfull \mdist{\prob{0}{0}{Q}\pair{Q_{0}}{\longmeasone{r_1}{r_2}{x}{x}}, \\
			\prob{1}{0}{Q}\pair{Q_{1}}{\longmeasone{r_2}{r_1}{x}{x}}} \\
		\sfull \mdist{\prob{0}{0}{Q}\prob{0}{2}{Q_0}\pair{Q_{0-0}}{(\blam f . f r_1) !(\lam x . x)}, \\
			\prob{0}{0}{Q}\prob{1}{2}{Q_{0--}}\pair{Q_{0-1}}{(\blam f . f r_1) !(\lam x . x)}, \\ \prob{1}{0}{Q}\prob{0}{1}{Q_{1}}\pair{Q_{10-}}{(\blam f . f r_2) !(\lam x . x)}, \\
			\prob{1}{0}{Q}\prob{1}{1}{Q_{1}}\pair{Q_{11-}}{(\blam f . f r_2) !(\lam x . x)}} \\
		\sfull \mdist{\prob{0}{0}{Q}\prob{0}{2}{Q_0}\pair{Q_{0-0}}{(\lam x . x) r_1}, \\
			\prob{0}{0}{Q}\prob{1}{2}{Q_0}\pair{Q_{0-1}}{(\lam x . x) r_1}, \\ \prob{1}{0}{Q}\prob{0}{1}{Q_{1}}\pair{Q_{10-}}{(\lam x . x) r_2}, \\
			\prob{1}{0}{Q}\prob{1}{1}{Q_{1}}\pair{Q_{11-}}{(\lam x . x) r_2}} \\
		\sfull \mdist{\prob{0}{0}{Q}\prob{0}{2}{Q_0}\pair{Q_{0-0}}{r_1}, \\
			\prob{0}{0}{Q}\prob{1}{2}{Q_0}\pair{Q_{0-1}}{r_1}, \\ \prob{1}{0}{Q}\prob{0}{1}{Q_{1}}\pair{Q_{10-}}{r_2}, \\
			\prob{1}{0}{Q}\prob{1}{1}{Q_{1}}\pair{Q_{11-}}{r_2}} \\
	$} \\
\end{example}





	


==> CF_Intro.tex <==
%!TEX root = Main_quantum.tex	
%\RED{TO DO:
%\begin{itemize}
%	\item define $I=\lambda x.x$
%	\item VALORIZE the difficulties and challanges. Which results are difficult and why? which solutions?
%\end{itemize}}


\section{Introduction }

Quantum computation is a model of computation in which one has access
to data coded on the state of objects governed by the law of quantum
physics. Due to the unique nature of quantum mechanics, quantum data
exhibits several non-intuitive properties~\cite{nielsen02quantum}: it
is non-duplicable, can exist in superposition, and reading the memory
is probabilistic. Nonetheless, the mathematical formalization is
well-established: the state of a quantum memory can be modeled as a
normalized vector in a Hilbert space.
%The
%basic unit of quantum information is the quantum bit ---whose
%semantics is a $2$-dimensional Hilbert space, and a quantum memory
%consisting of $n$ quantum bits corresponds to a Hilbert space of
%dimension $2^n$.

Knill's QRAM model~\cite{knill96conventions} proposes a generic interface for
interacting with such a quantum memory: it consists in uniquely
identified quantum registers, each holding one qubit. The interface
should make it possible to create and discard registers, and to apply
elementary operations on arbitrary registers.
%
Quantum algorithms are typically designed with a model akin to Knill's
QRAM: they consist in sequences of quantum operations, measurements
and classical processing. The control flow is purely classical, and in
general the behavior of the algorithm depends on the results of
past measurements.


\paragraph{Quantum operations.}
The basic unit of information in
quantum computation is a quantum bit or \emph{qubit}. The state of a single qubit
is a a normalized vector of the 2-dimensional Hilbert space $\CC^2$. We denote the
standard basis of $\CC^2$ as $\{\ket0,\ket1\}$, so that the general state of a single qubit can
be written as $\alpha \ket 0 + \beta \ket 1$, where $|\alpha|^2+|\beta|^2=1$

The basic operations on quantum states are unitary operations and measurements. A \emph{unitary operation} maps an n-qubit state to an n-qubit state, and is
described  by a \emph{unitary} $ 2^n \times  2^n $-matrix.
We assume that the language provides a  set of built-in unitary operations, including for example the \emph{Hadamard gate} $ H $ and the \emph{controlled not gate} $ \CNOT $:
%
\begin{minipage}{\textwidth}\scriptsize
	\begin{equation}
		H\defeq \dfrac{1}{\sqrt{2}}  \begin{pmatrix} 1 & 1\\ 1&-1\end{pmatrix}
		\quad\quad
		\CNOT \defeq 
		\begin{pmatrix}
			1 & 0& 0&0\\
			0 & 1& 0&0\\
			0 & 0& 0&1\\
			0& 0& 1&0\\
		\end{pmatrix}
	\end{equation}
\end{minipage}
\emph{Measurement}  a acts as a projection. When a qubit $\alpha \ket 0 + \beta \ket 1$ is measured, the 
observed outcome is a classical bit: either  $0$ or  $1$,  with 
probabilities $|\alpha|^2$   and $|\beta|^2$, respectively. 
Moreover, the state of the qbit collapses to $\ket 0$ (resp. $\ket 1$) if $0$ (resp. $ 1$) was observed.


\paragraph{Quantum $\lambda$-calculi} \cite{SelingerValiron, LagoMasiniZorzi, LagoMZ09, ArrighiD17,   pagani2014applying,popl17}  
\todoc{ADD MORE REFERENCE HERE (the more the better...)}
offer a formal setting for the foundation of quantum programming
languages. Akin to other extensions of lambda-calculus with
probabilistic~\cite{xxx} or non-deterministic behavior~\cite{xxx},
quantum lambda-calculi extend the regular lambda-calculus ---core of
functional programming languages--- with the interface to manipulate a
quantum memory. Due to the properties of the quantum memory, quantum
lambda-calculi should handle non-duplicable data and probabilistic
behavior.

\paragraph{No-cloning and linearity.}
In the litterature, non-duplicable data is usually captured with tools coming
from linear logic. The first
approach~\cite{selinger2006lambda,pagani2014applying,popl17} consists
in using types, imposing all functions to be linear by default and
with the use of a special type $!A$ to explicitely pinpoint duplicable
objects of type $A$. The other approach works with an
untyped~\cite{LagoMZ09,LagoMasiniZorzi}, but with a special term
construct ``$!$'' and validity constraints to forbid the duplication of
qubits.



\paragraph{Probabilistic behaviour: flipping a quantum coin.} Measurement makes the reduction probabilistic. Let us flip a fair quantum coin. In the examples below, $I \defeq \lam x.x$. 

\begin{example}[Fair quantum coin] The  term $L$ below produces a  qbit  in state $\frac{\sqrt{2}}{2}(\ket 0 + \ket 1)$ 
	by creating 	 a fresh qbit in state  $\ket 0$  ($\new$), and applying  the Hadamar  gate $H$. Measuring this qbit amounts to flipping  a fair coin, since the result is $\ket 0 $ or  $ \ket 1 $, with equal probability $\two$. 
		\[%L\defeq \texttt{ if }  \texttt{ meas}(H \new) \texttt{ then }  \true \texttt{ else } \false \quad
		  L \defeq \texttt{ if }  \texttt{ meas}(H \new) \texttt{ then }  I \texttt{ else } \Omega   \]
Observe that the term then  either stops with output I, or it diverges. That is, $L$ terminates with probability $\two$. 

\end{example}

\paragraph{... and the recursive quantum coin.}  %repeatedly



Untyped lambda calculus allows to encode recursive behaviour, giving to  programs rich expressiveness, but raising extra challenges, because   \textit{termination}  become probabilistic. 
A program may terminates \emph{with probability} $1$, but only at the limit (\emph{almost sure termination}).  A simple example suffices to illustrate this point. 



\begin{example}[Flipping a quantum coin, cont.]\label{ex:coin_cont} 
	Consider a quantum process  that flips a  coin, by creating a fresh qbit and measuring it. If the result is head ($\ket{0}$), the process stops , with output the value  $I$. If the result is tail ($\ket{0}$), it repeats.
%	Consider a program that	flips a quantum coin (by performing a measurement), returns a fresh qubit
%	on head ($\ket 0$) and repeats on tail ($\ket 1$). 
	In mock-up ML: 
	\[R\defeq  \mathtt{letrec} \: f  x =    \big(\ite{(\mathtt{meas} \; x)}{I}{f(H \new)}\big )   \;\mathtt{in}\;f (H \new)\]
%	where the if test 	performs a measurement on the qubit x. 
	%
%	where \textit{new} creates a fresh qubit in state $\ket 0$ and where the if test
%	performs a measurement on the qubit x. Note how the measure of
%	H new amounts to tossing a fair coin: H new produces  $\frac{\sqrt{2}}{2}$
%	Measuring gives $\ket 0$ or $\ket 0$ with equal  probability $\two$
%
\end{example}
  After $n$ iterations, the program $R$ is in   normal form with probability 
$\two + \frac{1}{2^2} + \dots + \frac{1}{2^n}$. % $\sum_{k:1}^n \frac{1}{2^k}$.
Even  if  the   termination probability is $1$, that degree of certitude 
is   not reached in a finite number of steps, but  \emph{as a limit}.
%\emph{Only at the limit} this computation terminates with probability $1$.

\Cref{ex:coin_cont}  will be our leading example; we formalize it in \Cref{ex:coin_formal}.

\paragraph{The operational semantics of quantum programs}
As it is customary for side effects, the probabilistic behavior
is dealt by fixing  an  \emph{evaluation strategy}. This is needed as, for
instance, duplicating a coin and using the result is not the same
thing as duplicating the coin and tossing it twice. Following what has
been done for functional languages with side-effects, the first 
evaluation strategy for quantum
lambda-calculi~\cite{selingervaliron,pagani2014applying,popl17} has
been a deterministic call-by-value strategy: an argument is reduced to a value
before being passed to a function.

One aspect that has been seldom examined is however the
\emph{properties} of the \emph{general reduction} associated to
quantum lambda-calculi. 
%


\paragraph{Evaluation strategy vs. general rewriting.}

Although programming languages based on $\lambda$-calculus
usually implement a specific \emph{evaluation strategy}, the
$\lambda$-calculus has a richer reduction theory, which 
provides a  \emph{sound framework for reasoning
	about programs transformations}, such as compiler
\emph{optimizations} or \emph{parallel implementations}, and a base on which to reason about program equivalence. 


 As
pioneered  by Plotkin in \cite{PlotkinCbV}, standardization allows to bridge
between the \emph{general rewriting} (where programs transformation can be
studied), and a specific \emph{evaluation strategy}, which implements the execution of 
an idealized programming language. 





Summing up, for  programming languages, there are  two kinds of term rewriting: run-time rewriting (“evaluation”) and compile-time rewriting  (programs transformations).
We see in this light  the 
 two fundamental operational  properties of $\lam$-calculi are
Confluence and Standardization. The former guarantees that normal
forms are unique, the latter that if a normal form exists, there is a
strategy which is guaranteed to compute it (normalization). 



% \cite{carraro2014semantical} defines a call-by-value lambda-calculus
% a-la Plotkin and adds two commuting rules, as dal-Lago. It features a
% lot of good properties, among which
% standardization~\cite{guerrieri2015standardization}.


\paragraph{A rewriting theory for quantum computation}
In the context of quantum lambda-calculi, the only line of research
discussing  \emph{rewriting} (rather then fixing a deterministic strategy) has been pursued by Dal Lago
\textit{et al.}~\cite{LagoMasiniZorzi,LagoMZ09}: working with an
untyped quantum lambda-calculus, they present confluence results, and also a form of 
 standardization, but only for the sub-language without
measurement\cite{LagoMZ09} ---and therefore without the probabilistic
behavior.

%\textcolor{red}{With a probabilistic behavior, the question of standardization is tied
%to the problem of termination. Consider \Cref{ex:coin} If it is non-terminating, we can
%nonetheless say that it does, \emph{at the limit}: we can say that it
%converges to $I$ with probability $I$, modulo an infinite reduction
%sequence. In this context, what does a standardization result mean?}



In this paper we study not only confluence, but also
\emph{standardization and normalization} for a  quantum $\lambda$-calculus featuring \emph{measurement}, and where $\beta$ reduction (the engine of $\lambda$-calculus) is fully unrestricted. 
 

Recent advances  in the literature of probabilistic and monadic  rewriting  give  us a way to tackle this task with a formalism and powerful techniques which were not available a decade ago. 
Still, quantum rewriting is \emph{more challenging} than probabilistic rewriting, because we need to manage the states of the quantum memory. 
The design of the language  is also  delicate, as we need to control duplication of qbits while allowing the full power of $\beta$ reduction.



\subsection{Setting the scene: the rewriting ingredients}
We conclude with a more detailed (but still informal) look at two key elements:   the  $\lambda$-calculus we adopt, and   what standardization results are about.

\paragraph{Untyped quantum $\lam$-calculus. }


%\subsection{Simpson's linear $\lam$-calculus}

Our  quantum  calculus is built on
top of Simpson's  calculus $\Lambda^!$ \cite{Simpson05},  a variant  of  untyped $\lam$-calculus inspired by Girard's  Linear Logic \cite{Girard87}. In this choice, we follow    \cite{LagoMasiniZorzi, LagoMZ09, popl17}.
 Indeed, the fine control
of duplication which $\Lambda^!$ inherits from linear logic makes it  an ideal base for quantum computation.

%

The Bang operator $!$ plays the role of a marker for non-linear management: duplicability and
discardability of resources.
Abstraction is refined into linear abstraction $\lam x.M$ and  non-linear abstraction $\lam!x.M$. The latter allows duplication of the argument, which is required  to be suspended as thunk  $!N$, behaving as the $!$-box of linear logic.







\begin{example}[duplication, or  not]\label{ex:duplicating}
	$(\lambda x.  Hx) (\new) $ is a valid term, but $ (\lambda x.  \tuple{x,x}) (\new) $ which would duplicate the qbit  created by $\new$ is not. Instead, we can validly write %$ (\blam x.  \tuple{x, x}) (! \new) $, 
	$ (\blam x.  \CNOT \tuple{Hx, x})( !\new)  $
	which thunks  $\new$ and then duplicate it, yielding 
	$ \CNOT \tuple{H\new, \new}  $. This term produces \emph{an entangled pair} of qbits.
\end{example}



In our  paper, as well as in \cite{LagoMasiniZorzi, LagoMZ09, popl17}, surface reduction (\ie, no reduction is allowed in the scope of the $!$ operator) is the key ingredient to allow for the coexistence
of quantum bits with duplication and erasing.
Unlike previous work however, in our setting 
 $\beta$ reduction ---the engine  of $\lambda$-calculus--- is  unconstrained. We  prove that only quantum
operations needs to be surface, making ours a conservative extension of the  usual  $\lambda$-calculus, with its  full power.

\paragraph{Call-by-Value... or rather,  Call-by-Push-Value.}
The reader may have recognized that reduction in our calculus follows the  Call-by-Push-Value paradigm, with the Bang operator \emph{thunking} a computation. In fact, 
Simpson's calculus \cite{Simpson05}, more precisely the fragment  without linear
abstraction, is essentially an untyped version of Call-by-Push-Value, and 
it has  been extensively studied   in the literature of Linear Logic also	with the name  of \emph{Bang calculus}
\cite{EhrhardGuerrieri16,GuerrieriManzonetto18, BucciarelliKRV23}, 
as a unifying framework which subsumes 
both Call-by-Name (CbN) and Call-by-Value(CbV) calculi. 


\paragraph{A taste of  Standardization and Normalization:  pure  $\lambda$-calculi.}
\begin{table}[tb]
	\centering
	\begin{tabular}{|l|l|l|}
		\hline
		\textbf{Call-by-name $\lambda$-calculus}
		& \textbf{Call-by-value $\lambda_v$-calculus}
		& \textbf{Linear $\lambda_!$-calculus}
		\\\hline
		General reduction: $(\to_\beta)$
		& General reduction: $(\to_{\beta_v})$
		& General reduction: $(\to_{\beta_!})$
		\\
		Evaluation: head ($\to_h$)  %\weak-head
		& Evaluation: weak-left ($\to_l$)
		& Evaluation: surface ($\to_s$)
		\\
		\emph{1. Head factorization}: 
		& \emph{1. Weak-left factorization}:
		& \emph{1. Surface factorization}:
		\\
		\quad $M\to^*_\beta N$ iff $M\to^*_h \cdot\to^*_{\neg h} N$
		& \quad $M\to^*_{\beta_v} N$ iff $M\to^*_l \cdot\to^*_{\neg l} N$
		&\quad  $M\to^*_{\beta_!} N$ iff $M\to^*_s \cdot\to^*_{\neg s} N$
		\\
		\emph{2. Head normalization}: 
		& \emph{2. Convergence to a value}:
		& \emph{2. Surface factorization}:
		\\
		\quad $M\to^*_\beta H$ iff $M\to^*_h H'$
		&\quad $M\to^*_{\beta_v} V$ iff $M\to^*_l V'$
		&\quad  $M\to^*_{\beta_!} S$ iff $M\to^*_s S'$
		\\\hline
	\end{tabular}
	\caption{Summarizing Standard Factorization and Normalization Results}
	\label{tab:fact-lc}
\end{table}




Termination and confluence concern the existence
and the uniqueness of normal forms, which are the results of a computation.
Standardization and normalization are  concerned with   \emph{how to compute} a given outcome. For example, is there a strategy which guarantees termination, if possible? The desired  outcome is generally a specific kind of terms. 
In the classical theory of $\lambda$-calculus (\'a la Barendregt), the terms of interest are  \emph{head normal forms}. In the  Call-by-Value approach, the terms of computational interest are values.


%For example, "is there a specific strategy which is guaranteed to produce a normal form, if any exist?". 


 \emph{Classical $\lambda$-calculus.}
The simplest form of standardization is \emph{factorization}: any reduction sequence
can be re-organized so to first performing specific steps and then
everything else.
A 
paradigmatic example is the head factorization theorem of classical  $\lambda$-calculus 
(theorem 11.4.6 in \cite{Barendregt}):
every $\beta$-reduction sequence $M\to^*_\beta N$ can be 
re-organized/factorized so as to first reducing head redexes and then everything else---in symbols 
$M\to^*_h \cdot\to^*_{\neg h} N$.

A major  consequence is \emph{head normalization}, relating arbitrary  $\beta$ reduction with \emph{head} reduction, w.r.t. 
\emph{head normal forms},  the  terms of computational interest in classical $\lambda$-calculus. 
A term $M$ has head normal form ) if and only if head reduction terminates: 
\begin{center}
	$M\redb^* H (\text{hnf})$ $ \Leftrightarrow $ $M\hredb H' (\text{hnf})$
\end{center}

 \emph{Plotkin's Call-by-Value.}
This kind of results  takes  its full computational meaning in   Plotkin's \cite{PlotkinCbV}  Call-by-Value $\lambda$-calculus
The terms of interest are here \emph{values}. Plotkin relates arbitary $\beta$ reduction ($\to_{\beta_v}$) and the evaluation strategy $\to_l$ which only performs \emph{ left-weak} steps (no reduction in the scope of  abstractions), by establishing
\begin{center}
	$M\redbv^* V (\text{value})$ $ \Leftrightarrow $   $M\wredbv V' (\text{value})$
\end{center}
In words: the unconstrained  reduction ($\to_{\beta_v}$) returns  a value if and only if   the evaluation ($\to_l$)  strategy   returns a value.
%
The  proof relies on a factorization: 
$M\to^*_{\beta_v} N$ iff $M\to^*_l \cdot\to^*_{\neg l} N$.



 \emph{Simpson's pure calculus.} Standardization and Normalization results have been established by  Simpson also for   its linear calculus \cite{Simpson05}. Here,  the evaluation strategy is  \emph{surface reduction}, \ie no reduction is allowed in the scope of a $!$ operator. %Surface normal forms play a similar role to head normal forms, and to values in Call-by-Value.
%
%
%The fragment of Simpson's  linear $\lambda$-calculus \cite{Simpson05} without linear abstraction is known in the literature as Bang calculus. It is closely related to Levy's Call-by-Push-Value \cite{Levy99}, and it has extensively been studied   in \cite{EhrhardGuerrieri16,GuerrieriManzonetto18, BucciarelliKRV23}.


\noindent \emph{Summary.} The table in \Cref{tab:fact-lc} summarize the factorization and normalization result for $\beta$ reduction in the three calculi we have discussed.

%%% Local Variables:
%%% TeX-master: "Main_quantum.tex"
%%% End:







==> CF_Syntax.tex <==
%!TEX root = Main_quantum.tex	

\newcommand{\program}{program\xspace}
\newcommand{\Program}{Program\xspace}





\section{Untyped quantum $\lambda$-calculus} \label{sec:syntax}
%In this section, we define an untyped quantum  $\lambda$-calculus  on top of Simpson's $\Lambda^!$ . 

Quantum lambda-calculus is an idealization of functional quantum
programming languages: following Selinger and Valiron
\cite{SelingerValiron}, it consists of a regular $\lambda$-calculus
together with specific constructs for manipulating quantum data and
quantum operations. One of the problem consists in accomodating the
non-duplicability of quantum information: in a typed setting
\cite{SelingerValiron} one can rely on linear type system. In our
untyped setting, we instead base our language on Simpson's
$\lambda$-calculus \cite{Simpson05}, extended with constructs
corresponding to quantum data and quantum operations.

Because of entanglement, quantum data cannot easily be written inside
lambda-terms. A standard procedure \cite{SelingerValiron} relies on an
external memory with register identifiers used as placeholders for
qubits inside the lambda-term. As they stands for qubits, these
registers are taken as non-duplicable.

In the original quantum lambda-calculus \cite{SelingerValiron},
regular free variables of type qubit were used to represent
registers. In this work, being untyped we prefer to consider two kinds
of variables: regular term variables, and special variable, called
\emph{registers} and denoted by $r_i$ with $i\in \Nat$, corresponding
to the qubit number $i$ in the quantum memory. 
%
The language is also equipped with term constructs to manipulate
quantum information:
\begin{itemize}
\item $\new$ is a term reducing to a fresh qubit\footnote{%
    Unlike the original quantum $\lambda$-calculus
    \cite{SelingerValiron}, the term $\new$ is not a value: it
    literally evaluates to a qubit.%
}.
\item $\meas{r_i}{M_0}{M_1}$ corresponds to a destructive measurement
  of the qubit corresponding to the register $r_i$. The evaluation
  then \emph{probabilistically} continues as $M_0$ or $M_1$, depending
  on the measure being $\ket 0$ or $\ket 1$.
\item Assuming that the memory comes with a set of built-in unitary
  gates ranged over by letters $A, B, C$, the term $U_A$ corresponds
  to a function applying the gate $A$.
\end{itemize}

\subsection{Terms}

Formally, \emph{raw terms} $M, N, P, \dots$ are built according to the
following grammar.
\begin{align*}\label{terms}\tag{\textbf{terms} $\QLambda$}
  M,N,P  ::={} & x \mid {!M} \mid
          \lam x.M \mid
          \blam x.M \mid M N \mid r_{i} \mid U_{A} \mid 
          \new \mid \meas{P}{M}{N}
\end{align*}
where $x$ ranges over a countable set of \emph{variables}, $r_{i}$
over a disjoint set of \emph{registers} where $i\in \Nat$ is called
the \emph{identifier} of the register, and $U_{A}$ over a set of
build-in n-ary \emph{gates}.  In this paper, we limit the arity $n$ to
be $1$ or $2$.
%
Pairs do not appear as a primitive construct, but we adopt the
standard encoding, writing $\tpair{M}{N}$ as sugar for
$\termPair{f}{M}{N}$. We also use the shorthand
$\tuple{M_1, \dots,M_n}$ for $\tuple{M_1\tuple{M_2, \dots}}$.
%
The variable $x$ is bound in both $\lam x . P$ and $\blam x . P$. As
usual, we silently work modulo $\alpha$-equivalence.
%
Given a term of shape $\meas{P}{M}{N}$, we call $M$ and $N$ its
\emph{branches}.
%
As usual, the set of free variables of a term $M$ are denoted with
$\FV{M}$. The set of registers identifiers for a term $M$ is denoted
with $\Reg{M}$.


\begin{remark}\label{rem:pb-lin}
  Without any constraints, one can write terms such as
  $\pair{r_0,r_0}$ or $\lambda x.\pair{x,x}$. Both are invalid: the
  former since a qubit cannot be duplicated, the latter since
  $\lambda$-abstractions are meant to be linear in Simpson's calculus.
\end{remark}

\paragraph{Term validity.}
%
To answer the problem in Remark~\ref{rem:pb-lin}, we introduce the
notions of context, surface context, occurence and surface occurence.

A context is a term with a hole. We define general \emph{contexts}
where the hole can appear anywhere, and \emph{surface contexts} for
contexts where holes do not occur in the scope of a $\bang$ operator,
nor in the branches of a $\meas{-}{-}{-}$. They are generated by the
grammars
\begin{align*}\tag{\textbf{contexts}}
  \cc 
  ::= {}
  & \hole{~}  \mid M \cc \mid \cc M   \mid \lam x . \cc \mid  \blam x . \cc  
    \mid\meas{\cc}{M}{N} \mid  \\
  & \meas{M}{\cc}{N}\mid \meas{M}{N}{\cc}\mid{! \cc},
  \\
  \tag{\textbf{surface contexts}}
  \ss ::={} & \hole{~} \mid M \ss \mid \ss M   \mid \lam x . \ss \mid  \blam x . \ss 
              \mid \meas{\ss}{M}{N},
\end{align*}
%                          
where $\hole{~}$ denotes the \emph{hole} of the corresponding context. The
notation $\cc\hole{R}$ (or $\ss\hole{R}$) stands for the term where the only occurrence
of a hole $\hole{~}$ in $\cc$ (or $\ss$) is replaced with the term $R$,
potentially capturing free variables of $R$.

From contexts and surface context we define two notions of occurence.
The pair $(\cc, T)$ (resp. $(\ss, T)$) is an \emph{occurence}
(resp. \emph{surface occurence}) of $M$ whever $M = \cc\hole{T}$
(resp. $M=\ss\hole{T}$). By abuse of notation we refer to $T$ alone as
the occurence of $M$, being understood that it is within a given
context.

We can now define a notion of valid terms, agreeing with the quantum
principle of no-cloning as follows.

\begin{Def}[ Valid Terms, and Linearity]\label{def:validity}\rm
  A term $M$ is \textbf{valid} whenever
  \begin{itemize}
  \item no register occurs in $M$ more than once, and every
    occurrences of registers are surface;
  \item for every subterm $\lam x . P$ of $M$, $x$ is \emph{linear} in
    $P$, \ie $x$ occurs free exactly once in $P$ and, moreover, this
    occurrence of $x$ is surface.
  \end{itemize}
\end{Def}


\begin{remark}
  The validity conditions for registers and linear variables do not
  allow us to put registers inside branches. So for instance we cannot
  directly write terms such as
  $\lam z. \meas{r_0}{z\,(U_A\,r_1)}{z\,(U_B\,r_1)}$. One can however
  simulate such a behavior with a speciic encoding. We can for
  instance write a term behaviorally equivalent to the previous
  one  as follows:
  $(\blam f. f z r_1)\meas{r_0}{!(\lam u x.u(U_{A} x))}{!(\lam u
    x.u(U_{B} x)}$. 
\end{remark}


\subsection{Programs}\todoc{In the body we use the term \textbf{qubits state} for quantum memory state. Mention here?}\todoc{@C: convert qbit in qubit}

In order to associate quantum states to registers in lambda-terms, we
introduce the notion of program, consisting of a \emph{quantum memory}
and a lambda-term of $\QLambda$. A program is closed under permutation
of register identifiers.

The \emph{state} of one qubit is a normalized vector in
$\qstates=\Cmp^2$.  The \emph{state} of a quantum memory consisting of
$n$ qubits is a normalized vector
$\Q\in\qstates^n = (\Cmp^2)^{\otimes n}$, the $n$-fold Kronecker product
of $\qstates$. The size of $\Q$ is written $|\Q|\defeq n$.  We
identify a canonical basis element of $\qstates^n$ with a string of
bits of size $n$, denoted with $\ket{b_0{\ldots}b_{n-1}}$. A state
$\Q\in\qstates^n$ is therefore in general of the form
\(
\mem{Q} = \sum_{b_0,{\ldots}b_{n-1}\in\{0,1\}}\alpha_{b_0{\ldots}b_{n-1}}\ket{b_0{\ldots}b_{n-1}}.
\)
If $\sigma$ is a permutation of $\{0,\ldots n-1\}$, we define $\sigma(\Q)$ as
\(
\sigma(\Q) = \sum_{b_0,{\ldots}b_{n-1}\in\{0,1\}}\alpha_{b_0{\ldots}b_{n-1}}\ket{b_{\sigma(0)}{\ldots}b_{\sigma(n-1)}}.
\)





A \emph{raw program $\et$} is then a pair $\pair{\mem{Q}}{M}$, where
$\mem{Q} \in \qstates^{n}$ and where $M$ is a valid term such that
$\Reg{M}=\{0,\ldots,n-1\}$.  We call $n$ the size of $\mem{Q}$ and we
denote it with $\memsize{\mem{Q}}$. If $\sigma$ is a permutation over
the set $\{0..n-1\}$, the \emph{re-indexing} $\sigma(\et)$ of $\et$ is
the pair $\pair{\sigma(\Q)}{\sigma(M)}$ where $\sigma(M)$ is $M$ with
each occurence of $r_i$ replaced by $r_{\sigma(i)}$.

\begin{Def}[Program] \label{def:programs}\rm A \emph{program} is an equivalence class of raw programs
  under re-indexing. We identify programs with their representative
  elements. The set of all programs is denoted with $\States$.
\end{Def}

\begin{example}\label{ex:reindexing}
  The following two raw programs are equal modulo re-indexing:
  \( \pair {\ket \psi\otimes \ket \phi}{\tuple{r_0 ,r_1}} = \pair
  {\ket \phi\otimes \ket \psi}{\tuple{r_1, r_0}} \).  In both cases,
  $\ket\psi$ is the first qubit in the pair and $\ket\phi$ the second
  one. Re-indexing is agnostic with respect to entanglement, and we
  also have the raw program
  \(
    \pair {\alpha\ket{00}+\beta\ket{01}+\gamma\ket{10}+\delta\ket{11}}{\tuple{r_0 ,r_1}}
  \)
  being a re-indexation of the raw program
  \(
    \pair {\alpha\ket{00}+\gamma\ket{01}+\beta\ket{10}+\delta\ket{11}}{\tuple{r_1 ,r_0}}
  \): they are two representative elements of the same program.
\end{example}




\section{Operational Semantics}

%The intended behaviour of
%$\et = \pair{\frac1{\sqrt2}(\ket0+\ket1)}{\meas{r_0}{M}{N}}$ is to
%reduce to either $\et_0=\pair{\ket0}{M}$ or $\et_1=\pair{\ket1}{N}$,
% \emph{with equal  probability} $\frac12$. 
In order to define the operational semantics of the quantum lambda calculus, we need to formalize   probabilistic reduction.  We do so   by means of a rewrite system
over \emph{multi-distributions}, adopting the \emph{monadic}  approach  recently developed  in the literature of probabilistic rewriting (see \eg \cite{AvanziniLY20,  popl17, DiazMartinez17, Faggian22})  %Faggian22
Reduction is here   defined not simply on  programs, but on (monadic) structures representing probability distributions over programs, called \emph{multi-distributions}.

The operational semantics of the language is defined by first
specifying the probabilistic behavior of programs, then  lifting reduction 
to multidistributions of programs. 
%The latter is the target calculus, presented in Section~\ref{xxx}.






%


\subsection{Distributions and Multi-distributions.}

Let us recall the definition of (discrete) Probability Distributions, and then introduce the notion of multi-distribution.

\emph{\textbf{Probability Distributions.}}\label{notation:dist} Given    a countable set $\Omega$, a
function $\mu \colon\Omega\to[0,1]$ is a probability \emph{subdistribution} if 
$\norm \mu := \sum_{\omega\in \Omega} \mu(\omega)\leq 1$ (a \emph{distribution} if $\norm \mu=1$).
%With a slight abuse of language, we will use the term distribution  also for   subdistribution. 
Subdistributions allow us to deal with partial results.
%
We write  $\DST{\Omega}$ for the set
of   subdistributions on $\Omega$,  equipped with the pointwise order on functions:  $\mu \leq \rho$ if
$\mu (\omega) \leq \rho (\omega)$ for 
all $\omega\in \Omega$. 
$\DST{\Omega}$ has a bottom  element (the subdistribution $\zero$) and maximal elements (all distributions).
%


\emph{\textbf{Multi-distributions.}}\label{sec:multi} 
We use multi-distributions \cite{AvanziniLY20} to \emph{syntactically} represent distributions. %we  rely on the notion of multi-distribution  \cite{Avanzini}.
%
A \emph{multi-distribution} $\m=\mdist{q_i\et_i}_{ i\in I}$ on the set of programs $\Programs$   is a finite multiset of pairs of the 
form
$q_i \et_i$, with $q_i\in]0,1]$,  $M\in \Lambda$, and  $\sum_i q_i\leq 1$.
The set of
all multi-distributions on $\Programs$ is $\MQ$.
The sum of multi-distributions is noted  $+$.  
The product $q\cdot \m$ of a scalar $q$ and a multi-distribution $\m$ is
defined pointwise $q\mdist{p_i \et_i}_{\iI} := \mdist{(qp_i) \et_i}_{\iI} $. We   write $\mdist{\et}$ for   $\mdist{1 \et}$.



\subsection{The rewrite system  $\QQ$}

%The calculus $\Q$ is the rewrite system  $(\MQ, \Red)$ where    
%the relation $\Red\subseteq \MQ\times \MQ$ is defined in  

%The  \emph{calculus} $\PLambda^\cbv$ is the rewrite system  $(\MPLambda, \Red)$ where   
%$\MPLambda$ is the set of  \emph{multi-distributions} on $\PLambda$ and 
%the relation $\Red\subseteq \MDST{\PLambda}\times \MDST{\PLambda}$ is defined in  
%\Cref{fig:reductions} and \Cref{fig:lifting}.  

 $\QQ$ is the rewrite system  $(\MQ, \Red)$ where    
the relation $\Red\subseteq \MQ\times \MQ$ is monadically defined in two phases.
(\Cref{fig:rules}, \Cref{fig:steps} and \Cref{fig:lifting})
\begin{itemize}
	\item[I.] \textbf{ Programs reduction.} First, we define   \emph{one-step reductions} from programs to 
multi-distributions---for example 
\[ \et  \red 
\mdist{   \two \pair{\ket0}{M},   \two \pair{\ket 1}{N}} \quad \quad\mbox{ where }  \et \defeq \pair{\frac1{\sqrt2}(\ket0+\ket1)}{\meas{r_0}{M}{N}}  \]


\item[II.] \textbf{ Lifting.} Then, we \emph{lift} the definition of reduction to a binary relation on $\MQ$,  in the natural way
---so for instance, for the same $\et$ as above  
\[ \mdist{\two \et, \two \pair {\Q}{(\lambda x.xx)F}}  \red 
\mdist{   \frac{1}{4} \pair{\ket 0}{M},   \frac {1}{4} \pair{\ket 1}{N},  \two \pair {\Q}{FF}} \]

\end{itemize}

Let us see the details.

%\begin{enumerate}
%	\item  The reduction steps
%	$\redb,\redq\subseteq \States \times \MQ$ are defined  in 	\Cref{fig:steps} as the  contextual closure of the basic rules
%	$\mapsto_{\beta}$ and $\mapsto_{q}$, which are defined in \Cref{fig:rules}.
%	Observe that  while the $\beta$ rules 
%	are closed under
%	arbitrary  contexts $\cc$,      the quantum rules are closed only under surface  
%	contexts (no reduction inside a $!$-box, nor in the branches of $\meas---$). 
%	The relation  $\red$  is the union $\redb \cup \redq$. 
%	
%
%	\emph{Surface  reduction} is  $\sred \eq \sredb \cup \redq$, 	where we write $\sredb$ for  the closure of $\beta$ under surface  context $\ss$.
%	A $\red$-step which is not surface is noted $\nsred$.
%	%	 \emph{Surface  reduction.}  The  restriction of the beta rules  to closure  under surface  context is denoted $\sredb$. 	Surface reduction  $\sred$ (\Cref{fig:surface_steps}) is  
%	%	the union of the surface  reductions $\sredb \cup \redq$. A $\red$-step which is not surface is noted $\nsred$.
%	
%	
%	\item 
%	The lifting of a relation
%	$\red_r \subseteq  \States \times \MQ$ to a reduction on multi-distribution is defined  in 
%	\Cref{fig:lifting}. 
%	In particular, 
%	$\red, \redb,\redq, $ lift to 
%	$\Red,\Redb,\Redq$, respectively.
%	%	In particular, 
%	%	$\red, \redb,\redq, \sred,\nsred$ lift to 
%	%	$\Red,\Redb,\Redq, \sRed, \nsRed$, respectively.
%	Similarly, $ \sred,\nsred$ lift to 
%	$\sRed, \nsRed$. 
%\end{enumerate}


\paragraph{I. Programs reduction.}
We first define the reduction of a program $\et$ to a multi-distribution.
The operational behavior of $\et$ is  given by 
beta reductions, denoted with $\redb$, and specific rules for handling
quantum operations---the corresponding reduction is denoted with
$\redq$.  


The reduction steps
$\redb,\redq\subseteq \States \times \MQ$ are defined   as the  contextual closure (\Cref{fig:steps}) of the root rules
$\mapsto_{\beta}$ and $\mapsto_{q}$, which are given in \Cref{fig:rules}.
The relation  $\red$  is the union $\redb \cup \redq$. 

\begin{itemize}
	\item \textbf{The root rules} are given in  \Cref{fig:rules}.  We call \emph{redex} the term on the  left-hand side of a rule.  Beta rules come in two flavors, the linear one (b), which does not allow for duplication,
	and the non-linear one (b!), which possibly duplicate boxes (\ie terms of shape $!M$). 
	
	Quantum rules act on the qubits state, exactly implement the operation which we  had informally described in \Cref{sec:syntax}.  Notice  that the rule  $  (m) $ has a probabilistic behaviour. The qubit which has been measured can be discharged (as we actually do).
	\begin{remark}[Reindexing]
		As in \cite{SelingerValiron}, reduction is defined on programs, which are equivalence classes. We define the rules on a convenient representative. For example,  in  \Cref{fig:rules} rule ($u_1$) reduces the redex $U_Ar_0$. Modulo reindexing, the same rules can be applied to any other register $U_Ar_j$ ($j\in \Nat$).
	\end{remark}
	\item \textbf{The contextual closure of the rules} is in \Cref{fig:steps}.  	Observe that  while the $\beta$ rules 
	are closed under
	arbitrary  contexts $\cc$,   while   the quantum rules are restricted  to surface 
	contexts  $\ss$ (no reduction inside a $!$-box, nor in the branches of $\meas---$). This constraints guarantee that qubits are neither duplicated nor delated.
	
	
\end{itemize}






\paragraph{II. Lifting.}
	The lifting of a relation
	$\red_r \subseteq  \States \times \MQ$ to a reduction on multi-distribution is defined  in 
	\Cref{fig:lifting}. 
	In particular, 
	$\red, \redb,\redq, $ lift to 
	$\Red,\Redb,\Redq$, respectively.
	%	In particular, 
	%	$\red, \redb,\redq, \sred,\nsred$ lift to 
	%	$\Red,\Redb,\Redq, \sRed, \nsRed$, respectively.
	


















%
%\begin{align*}
%b \quad  & \pair{\mem{Q}}{(\lam x . M)N} \mapsto_{\beta} \mdist{\pair{\mem{Q}}{M
%			\subs{x}{N} } }\\
% !b \quad & \pair{\mem{Q}}{(\blam x . M) !N } \mapsto_{\beta} \mdist{\pair{\mem{Q}}{M \subs{x}{N}}}\\
%\end{align*}
%\begin{align*}
%	(n) \quad& 
%	\pair{\Q}{\new}
%	\mapsto_{q}
%	\mdist{\pair{\Q\otimes\ket{0}}{r_{n}}} 
%	\mbox{  where $|\Q| = n$}\\
%	(m)\quad &
%	\pair{\Q}{\meas{r_{n}}{M}{N}}
%	\mapsto_{q}
%	\mdist{ |\alpha_0|^2\pair{\Q_0}{M},|\alpha_1|^2\pair{\Q_1}{N}}\\
%	&	\mbox{ where $\Q= \alpha_0\Q_0\otimes\ket0 + \alpha_1\Q_1\otimes\ket1$ and $Q$ has $n+1$ qubits}\\
%	%
%	(u_1) \quad& \mbox{for   $A$    unary operator:}\\
%	&\pair{\Q}{U_{A}\,r_{0}}
%	\mapsto_{q}
%	\mdist{\pair{\Q'}{r_{0}}}
%	\mbox{ where $\Q'$ is $(A\otimes\text{Id})\Q$}\\
%	%
%	( u_2 ) \quad& \mbox{ for $A$   binary operator:}\\
%	&\pair{\Q}{(U_{A}\,\tpair {r_{0}}{r_{1}}}
%	\mapsto_{q}
%	\mdist{\pair{\Q'}{\tpair {r_{0}}{r_{1}} }}
%	\mbox{ where
%		$\Q'$ is $(A\otimes\text{Id})\Q$.}
%\end{align*}



\begin{figure}[tb]\centering
\footnotesize{
  \begin{tabular}{l|l}
  \textbf{$\beta$ rules} &    \textbf{Quantum rules}\\[2pt]
 %
 $\begin{array}{ll}
 	(b)   & \pair{\mem{Q}}{(\lam x . M)N} \mapsto_{\beta} \mdist{\pair{\mem{Q}}{M
 			\subs{x}{N} } }\\
 	(!b)  & \pair{\mem{Q}}{(\blam x . M) !N } \mapsto_{\beta} \mdist{\pair{\mem{Q}}{M \subs{x}{N}}}\\
 \end{array}$ %\\[4pt]  % \hline\\
&
  $  \begin{array}{ll}
    	(n) & 
    	\pair{\Q}{\new}
    	\mapsto_{q}
    	\mdist{\pair{\Q\otimes\ket{0}}{r_{n}}} 
    	\mbox{  where $|\Q| = n$}\\
    	(m) &
    	\pair{\Q}{\meas{r_{n}}{M}{N}}
    	\mapsto_{q}
    	\mdist{ |\alpha_0|^2\pair{\Q_0}{M},|\alpha_1|^2\pair{\Q_1}{N}}\\
    	&	\mbox{ where $\Q= \alpha_0\Q_0\otimes\ket0 + \alpha_1\Q_1\otimes\ket1$ and $Q$ has $n+1$ qubits}\\
    	%
    	(u_1) & \mbox{for   $A$    unary operator:}\\
    	&\pair{\Q}{U_{A}\,r_{0}}
    	\mapsto_{q}
    	\mdist{\pair{\Q'}{r_{0}}}
    	\mbox{ where $\Q'$ is $(A\otimes\Id)\Q$}\\
    	%
    	( u_2 ) & \mbox{ for $A$   binary operator:}\\
    	&\pair{\Q}{(U_{A}\,\tpair {r_{0}}{r_{1}}}
    	\mapsto_{q}
    	\mdist{\pair{\Q'}{\tpair {r_{0}}{r_{1}} }}
    	\mbox{ where
    		$\Q'$ is $(A\otimes\Id)\Q$.}
    \end{array}$
%
%
  \end{tabular}
}
  \caption{Basic rules $(\mapsto)$}
  \label{fig:rules}
  \vskip 8pt
  %
	\begin{tabular}{l|l}
			\textbf{$\beta$ steps} &\textbf{ Quantum steps} \\[2pt]
			$\infer{\pair \Q{\cc \hole {M} }\redb \mdist{\pair \Q {\cc\hole
						{M'} }}}{\pair \Q M\mapsto_{\beta} \mdist{\pair \Q {M'}}}$
		&
		$	\infer{  \pair{\Q}{\ss\hole M} \sredq \mdist{p_i \pair{\Q_i}{\ss\hole{M_i}}} }
			{ \pair \Q M \mapsto_{q}
				\mdist{p_i \pair {\Q_i} {M_i}}}$
	\end{tabular}
\\[6pt]
	$\red~:=~\redb \cup \sredq$
	\caption{Contextual closure of basic rules:  $(\red)$}
	\label{fig:steps}
\end{figure}


\paragraph{Reduction Sequences.}%\label{def:sequence}
A $\Red$-sequence (or \emph{reduction sequence}) from $\m$ is a
sequence $\m=\m_0,\m_1,\m_2,\dots$ such that $\m_{i}
\Red\m_{i+1}$ for every $i$.
%
We write
$\m_0\Red^*\m$ to indicate the existence of a finite reduction sequence from $\m_0$, and $\m_0\Red^k
\m$ to specify the number $k$ of $\Red$-steps. Given a program  $\et$ and $\m_0=\mdist \et$, the sequence $\m_0 \Red
\m_1\Red\cdots$ naturally models the evaluation of $\et$; each $\m_k$ expresses the
``expected'' state of the system after $k$ steps.


\paragraph{Examples.}Let us  see 
  the definitions at work in  a few examples. We first formalize  the recursive program from   \Cref{ex:coin_cont}.
   Recall that $H$ is the Hadamar gate, and $I\defeq \lam x.x$. 
\begin{example}[Flipping the quantum coin]\label{ex:coin_formal} The program in  \Cref{ex:coin_cont} can be written as $\et \defeq \pair{~\ket{}}{\Delta ! \Delta}$, where  $\ket{}$ is just the   empty memory and 
	$\Delta \defeq \blam x . \meas{H \new}{I}{x ! x}$.  A reduction from $\et$ behaves as follows. At every reduction step, we underline the redex.
	\begin{flalign}
		\mdist {\pair{~\ket{}}{\underline{\Delta ! \Delta}}} &\Red
		\mdist{\pair{~\ket{}}{\meas{U_H \underline{\new}}{I}{\Delta ! \Delta}}} 
		\Red \mdist{\pair{~ \ket{0}}{\meas{\underline{U_H r_0}}{I}{\Delta ! \Delta}}}  \\
	&	\Red \mdist{\pair{~ \frac{\sqrt{2}}{2}(\ket{0}+\ket 1)}{\underline{\meas{ r_0}{I}{\Delta ! \Delta}}}}  \Red
		\mdist{\two \pair{\ket{}}{I} , \two \pair {\ket{}}{\Delta ! \Delta}}\\
		&\Red \dots  \Red \mdist{\two \pair{\ket{}}{I} , \frac{1}{4} \pair {\ket{}}{I},  \frac{1}{4} \pair {\ket{}}{\Delta ! \Delta}
		\Red \dots }
	\end{flalign}
	Notice that the first  step is a $\bbeta$ reduction. The reduction of $\new$ allocates a fresh qubit  in the memory, corresponding to the register $r_0$. The redex  $U_H r_0$ applies the Hadamar gate $H$ to that qubit. The last reduction performs \emph{measurement}, yielding a probabilistic outcome.
\end{example}


\begin{example}[Entangled pair]\label{ex:entangled} Let  $\et \defeq \pair{\ket{}}{\letin{\tuple{x,y}}{U_\CNOT \tpair{U_H \new}{\new}}{\meas{y}{I}{I}x}}$ (where $\leti \tuple{x,y} \dots$ is sugar for an  opportune encoding). This program produces an entangled pair of qubits (notice how  $\CNOT$ is applied to a pair of registers) and then measures one of the qubits. Let us formalize its  behaviour:
	\begin{flalign}\mdist{ \et}&\sRed^* \mdist{\pair{\hq \otimes \ket 0}{\letin{\tuple{x,y}}{\underline{U_\CNOT \tpair{r_0} {r_1}}}{\meas{y}{I}{I}x}} }\\
		& \sRed \mdist{\pair { \frac{\sqrt{2} }{2} \ket{00} + \frac{\sqrt 2}{2} \ket {11} }
			{\letin{\tuple{x,y}}{\tpair{r_0} {r_1}}{\meas{y}{I}{I}x}} }\\
		& \sRed^* \mdist{\pair { \frac{\sqrt{2} }{2} \ket{00} + \frac{\sqrt 2}{2} \ket {11} }
			{{\meas{r_1}{I}{I} r_0}} }
		 \sRed \mdist{\two \pair { \ket{0}}{I r_0} , \two \pair { \ket{1}}{I r_0}   }
	\end{flalign}

\end{example}



\begin{figure}
		{\footnotesize 
			\begin{minipage}[c]{0.6\textwidth}
				$
				\dfrac{}{\mdist{\et}\Red \mdist{\et}} \quad 
				\dfrac{\et\red\m}{\mdist{\et}\Red \m} \quad   
				\dfrac{(\mdist{\et_i} \Red \m_i)_{\iI} }{ \mdist{p_{i}\et_{i}\mid i\in I} \Red  \sum_{\iI} {p_i \!\cdot \m_i}} 
				$  	
				\caption{Lifting of $\red$}\label{fig:lifting}
	\end{minipage}}
\end{figure}

\condinc{}{
\begin{figure}
	\fbox{	
		{\footnotesize 
			\begin{minipage}[c]{0.6\textwidth}
				$
				\dfrac{}{\mdist{\et}\Red \mdist{\et}} \quad 
				\dfrac{\et\red\m}{\mdist{\et}\Red \m} \quad   
				\dfrac{(\mdist{\et_i} \Red \m_i)_{\iI} }{ \mdist{p_{i}\et_{i}\mid i\in I} \Red  \sum_{\iI} {p_i \!\cdot \m_i}} 
				$  	
				\caption{Lifting of $\red$}\label{fig:lifting}
				\vskip 4pt
				%
				{	$
					\dfrac{\et\not \red}{\mdist{\et}\full \mdist{\et}} \quad 
					\dfrac{\et\red\m}{\mdist{\et}\full \m}  \quad   
					\dfrac{(\mdist{\et_i} \full  \m_i)_{\iI} }{ \mdist{p_{i}\et_{i}\mid i\in I}\full  \sum_{\iI} {p_i \!\cdot \m_i}} 
					$}\caption{Full lifting of $\red$ }\label{fig:lifting_full}
	\end{minipage}}}
\end{figure}
}




%\paragraph{Technical properties.}
%The  restriction of  $\redq$ to surface contexts is necessary to respect the linearity of quantum computation, avoiding duplication or deletion of qubits.
%Validity of terms is preserved.
%\begin{fact}If $M$ is a valid term,  and $\pair \Q M \red \mdist{\pair{ \Q_i} {M_i}}$, then $M_i$ is a valid term.
%\end{fact}
%
%
%We will freely use the following   closure property, which is  immediate by  definition of context and  surface context.
%\begin{fact}[Closure]\label{fact:closure}
%	\begin{align*}
%		\infer[1.]{  \pair{\Q}{\ss\hole M} \redx{q} \mdist{p_i \pair{\Q_i}{\ss\hole{M_i}}} }
%		{ \pair \Q M \redx{c}
%			\mdist{p_i \pair {\Q_i} {M_i}} }   
%		\quad\quad
%		\infer[2.]{\pair \Q{\cc \hole {M} }\redb \mdist{\pair \Q {\cc\hole
%					{M'} }}}{\pair \Q M\redb \mdist{\pair \Q {M'}}}
%	\end{align*}
%	Surface closure (point 1.) also holds with $\redb$ in place of $\redq$.
%\end{fact}



\paragraph{Validity.}
Validity of terms is preserved.
\begin{fact}If $M$ is a valid term,  and $\pair \Q M \red \mdist{\pair{ \Q_i} {M_i}}$, then $M_i$ is a valid term.
\end{fact}
Notice that the  restriction of  $\redq$ to surface contexts is necessary to respect the linearity of quantum computation, avoiding duplication or deletion of qubits.



\subsection{Surface reduction and surface normal forms}
% Following Felleisen \cite{Felleisen'88},  general reduction  and evaluation  can be defined 	as the closure of   
% reduction rules under arbitrary and evaluation contexts, respectively.


So far, we have defined a very liberal  notion of reduction, in which $\beta$ is  unrestricted---it can validly  be performed even inside a $!$-box.
What shall we adopt as evaluation strategy?


In the setting of calculi based on linear logic, as Simpson's calculus \cite{Simpson05} and the Bang calculus \cite{EhrhardG16}, the natural candidate is 
 \textbf{surface reduction}.  The restriction of $\beta$ to surface contexts ($\sredx{\beta}$)  plays a  key  role akin  to that of  head reduction  in classical $\lambda$-calculus, yielding to similar factorization and normalization results which relate ($\redx{\beta}$) and $\sredx{\beta}$  (as recalled in \Cref{tab:fact-lc}).
 The terms of interest are   here 
 \textbf{surface normal forms}  (\snf), such as $x$ or $!M$.  They are the analog of values in Plotkin's Call-by-Value $\lam$-calculus and of head normal forms in classical $\lam$-calculus---such an analogy can indeed  be made precise \cite{EhrhardG16,GuerrieriManzonetto18, BucciarelliKRV23}\footnote{Yet another consequence  of Girard's translation of Call-by-Name and Call-by-Value $\lam$-calculi into Linear Logic.}.
 

In our setting, surface reduction and surface normal forms also play a privileged role.




%\paragraph{Surface  reduction} is  $\sred \eq \sredb \cup \redq$, 	where we write $\sredb$ for  the closure of $\beta$ under surface  context $\ss$.
%A $\red$-step which is not surface is noted $\nsred$.
%Similarly, $ \sred,\nsred$ lift to 
%$\sRed, \nsRed$. 
%
%A term $M$ is   $\red$-\textbf{normal} if there is no $\m$ such that $M\red\m$.; we also write $M\not\red$. 
%$M$ is a  \textbf{surface normal forms} (\snf) if $M\not\sred$. 
%%



\paragraph{Surface Reduction.} 
Surface steps   $\sred \subseteq \Programs \times \MQ$ (\Cref{fig:surface_steps}) are 
the union  $\sredb \cup \redq$ of quantum steps together with   restriction of the $\beta$ rules  to surface  context $\ss$.  
%
A program $\et$ is a  \textbf{surface normal form} (\snf) if $\et \not \sred$,  \ie  there is no surface reduction from $\et$. 
% Trivially, any program $\pair{\Q}{!M}$ is in surface normal form.


A $\red$-step which is not surface is noted $\nsred$. 
The  lifting  of $\sred,\nsred$ to relations  on multidistributions is  denoted $\sRed, \nsRed$ respectively.
% is defined as in  (\Cref{fig:lifting}).
\begin{remark}
Notice  that  $\nsred$ steps do not act on the qubits state,  since  they are  $ {\beta} $ steps.
\end{remark}


\paragraph{Strict lifting.} To guarantee normalization results (\Cref{sec:Asymptotic}), we will need a stricter form of lifting,
noted $\sfull$ (\Cref{fig:full_lifting}),  forcing  a reduction step to be  performed in each program of the multi-distribution $\r$, if a redex exists. Clearly $\sfull \subseteq \sRed$.

%
%We use the notation $\full$ for the  lifting of $\red$ in which 
%\emph{all} reducible terms in the underlying multidistributions
%are actually reduced according to $\sred$,
%
\begin{figure}[h]\centering
	\fbox{	
		{\footnotesize 
			\begin{minipage}[c]{0.6\textwidth}
				{	$
					\dfrac{\et\not \sred}{\mdist{\et}\sfull \mdist{\et}} \quad 
					\dfrac{\et\sred\m}{\mdist{\et}\sfull \m}  \quad   
					\dfrac{(\mdist{\et_i} \sfull  \m_i)_{\iI} }{ \mdist{p_{i}\et_{i}\mid i\in I}\sfull  \sum_{\iI} {p_i \!\cdot \m_i}} 
					$}\caption{Strict lifting of $\sred$ }\label{fig:full_lifting}
	\end{minipage}}}
\end{figure}
%
%\begin{figure}[h]\centering
%	\fbox{
	%		\begin{minipage}[c]{0.97\textwidth}			
		%			\[	\infer[]{\mdist{\et}\full_r  \mdist{\et}}{\et\not\red_r}\qquad \qquad
		%			\infer{\mdist{\et}\full_r \m}{\et\red_r\m}  \quad  \quad  \quad\quad\quad
		%			\infer{ \mdist{p_{i}\et_{i}\mid i\in I} \full_r ~\sum_{\iI}~ {p_i\cdot \m_i}} 
		%			{(\mdist{\et_i} \full_r \m_i)_{\iI} }\]
		%		\end{minipage}	
	%	}\caption{ Strict Lifting of $\red_r$ }\label{fig:full_lifting}
%\end{figure}

\begin{example} We will prove that  the strict lifting $\sfull$  guarantees to reach  \snf, if any exist.   This is obviously not the case for     $\sRed$-sequence 
{\footnotesize \begin{equation*}
	\mdist{\two I\new, \two \underline{(\blam x.x!x)  !(\blam x.x!x)}}
	\sRed \mdist{\two I\new, \two \underline{(\blam x.x!x)  !(\blam x.x!x)}}
	\sRed \mdist{\two I\new, \two \underline{(\blam x.x!x)  !(\blam x.x!x)}} \sRed\dots
\end{equation*}}
\end{example}


\cf{\paragraph{On the interest of surface normal forms.}
% A programs of shape $\pair{\Q}{S}$, with $S$  in surface normal form, guarantees   that  the qbits state $\Q$ is a \emph{stable} piece of information  (it will not further evolve in the computation).

What is the result of running a quantum program?
In general, since computation is probabilistic, the result of executing a program  will be a distribution over some  outcomes of interest. A natural choice are  programs of shape $\et \defeq \pair{\Q}{S}$, with $S$  in surface normal form, ensuring that at this point,
\emph{the qbits state $\Q$ is a \textbf{stable piece of information}}
(it will not further evolve in the computation). 	Indeed:
\begin{center}
  a program $\et\not\sred$ (in \snf) will no longer modify the qbits state. 
\end{center}
% ($\et$ has already produced the maximal amount of  data that it could possibly do.)

\begin{remark} Notice instead that a
	program  $\et \not\redx{q}$  (no quantum step is possible) 
	is not necessarily done  in manipulating the quantum memory.
	Further $\beta$ reductions may unblock further quantum steps. 
	Think of $ (\blam x.  \CNOT \tuple{Hx, x})( !\new)  $
	from  \Cref{ex:duplicating}.
\end{remark}
}


\input{01_Tables}
